ODIN: Obfuscation-based privacy preserving consensus algorithm for Decentralized Information fusion in smart device Networks

The large spread of sensors and smart devices in urban infrastructures are motivating research in the area of Internet of Thing (IoT), to develop new services and improve citizens' quality of life. Sensors and smart devices generate large amount of measurement data from sensing the environment, which is used to enable services, such as control power consumption or traffic density. To deal with such a large amount of information, and provide accurate measurements, service providers can adopt information fusion, which, given the decentralized nature of urban deployments, can be performed by means of consensus algorithms. These algorithms allow distributed agents to (iteratively) compute linear functions on the exchanged data, and take decisions based on the outcome, without the need for the support of a central entity. However, the use of consensus algorithms raises several security concerns, especially when private or security critical information are involved in the computation. This paper proposes ODIN, a novel algorithm that allows information fusion over encrypted data. ODIN is a privacy-preserving extension of the popular consensus gossip algorithm, that prevents distributed agents have direct access to the data while they iteratively reach consensus; agents cannot access even the final consensus value, but can only retrieve partial information, e.g., a binary decision. ODIN uses efficient additive obfuscation and proxy re-encryption during the update steps, and Garbled Circuits to take final decisions on the obfuscated consensus. We discuss the security of our proposal, and show its practicability and efficiency on real-world resource constrained devices, developing a prototype implementation for Raspberry Pi devices.

==> consensus.tex <==
\label{sec:consensus}
%\TODO{Let consider the consensus algorithm.}

The network is formally described by an undirected graph, whose vertices are the sensors and edges are the available communication links.
The set of nodes neighboring the $i^{th}$ node is denoted by ${\mathcal{N}}_i\subseteq[1,2,\dots,S]$, the sensor $i$ can communicate solely with sensors belonging to ${\mathcal{N}}_i$.
The adjacency matrix associated to the network graph is denoted by $A$, with $\left\{A\right\}_{ij}=1$ if $j\in {\mathcal{N}}_i$, otherwise $\left\{A\right\}_{ij}=0$. Since $j\in {\mathcal{N}}_i$ if and only if $i\in {\mathcal{N}}_j$, $A$ is symmetric, i.e., $A=A^T$.
Accordingly to the adjacency matrix a random averaging consensus matrix is defined $W(k)$ at time step $k$, the sensors update their state $y(k)$ accordingly to the following iterative rule 
\[
y(k) = W(k) y(k-1),
\]
where the initial state is given by the observation data $y(0)=\left[ {\mathcal{L}} (x_1), {\mathcal{L}} (x_2), \dots, {\mathcal{L}} (x_N) \right]^T$.
The consensus procedure has quite interesting properties, in particular under mild conditions (e.g. connectivity of the network graph) guarantees the convergence to the average of the initial vales $y_{i}(k) \rightarrow \bar{y} = \sum_{i=1}^N {{\mathcal{L}} (x_i)}/{N}$, $\forall i=1,\dots,N$, see details in~\cite{boyd-gossip-IT,Olfati-Saber,asymptotic-rc}.
For simplicity we focus here on the randomized gossip algorithm~\cite{boyd-gossip-IT} where at each consensus step a pair (or multiple pairs) of sensors exchange their information, say node $i$ and $j$ update their states at time $k$ accordingly to $y_{i}(k) = y_{j}(k) = \frac{y_{i}(k-1) + y_{j}(k-1)}{2}$, while the other nodes hold their previous value $y_{n} (k) = y_{n}(k-1), \forall n \neq i,j$. 



%Given a network composed by $N$ nodes $P_i$ whose connections at the step $k$ are described in the matrix $W_k$, the nodes are interested to apply the consensus algorithm on the input array $\mathbf{x^0}=[x_1^0,\ldots, x_N^0]$.
%In each step a node (randomly chosen) interacts with one of its neighbors (randomly chosen again) and updates their values computing the mean between the values they owns, i.e. $x_i^{k+1}=x_j^{k+1}=\frac{x_i^{k}+x_j^{k}}{2}$.


==> protocol_figure.tex <==
%\newcommand{\linesspace}{\\}
\newcommand{\linesspace}{\\[0.1cm]}
\protocolplot{} {Step $\tau$ of the secure consensus gossip protocol, involving agents $i$ and $j$. We assume that they previously updated their status with generic agents $k$ and $l$ respectively. All the operations are performed $\mod n$. Outputs of other agents at step $\tau$ are equal to their own inputs.} {pr:step} {
\scriptsize
$$
\begin{array}{lr}
{\mbox{\hspace*{1cm}Agent~}i} & {\mbox{Agent~}j\mbox{\hspace*{1cm}}} \\  %\small
\multicolumn{2}{c}{\hspace*{\textwidth}}\\
%
\multicolumn{2}{c}{\mbox{\bf Inputs:}}\linesspace
\begin{minipage}{0.45\textwidth}
{$n_i(\tau-1)+s_k(\tau-1)$, $\penc{s_k(\tau-1)}{k}$, $d_i(\tau-1)$} 
\end{minipage}
	& \begin{minipage}{0.45\textwidth}\begin{flushright}
		{$n_j(\tau-1)+s_l(\tau-1)$, $\penc{s_{_l}(\tau-1)}{l}$, $d_j(\tau-1)$}
	\end{flushright}\end{minipage}\linesspace
%	
\multicolumn{2}{c}{\mbox{\bf Outputs:}}\linesspace
\begin{minipage}{0.45\textwidth}
	{$n_i(\tau)+s_j(\tau)$, $\penc{s_j(\tau)}{j}$, $d_i(\tau)$} 
\end{minipage}
	& \begin{minipage}{0.45\textwidth}\begin{flushright}
		{$n_j(\tau)+s_i(\tau-1)$, $\penc{s_i(\tau)}{i}$, $d_j(\tau)$}
	\end{flushright}\end{minipage}\linesspace
%
\multicolumn{2}{c}{\mbox{\bf Protocol:}}\linesspace
r_i(\tau), s_i(\tau) \leftarrow_R \Z_N; & r_j(\tau), s_j(\tau) \leftarrow_R \Z_N;\linesspace
%\mbox{compute }\enc{n_i(\tau-1)+s_k(\tau-1)+r_i(\tau)}{j}; & \mbox{compute }\enc{n_j(\tau-1)+s_{_l}(\tau-1)+r_j(\tau)}{i};\linesspace
\mbox{compute }n_i(\tau-1)+s_k(\tau-1)+r_i(\tau); & \mbox{compute }n_j(\tau-1)+s_{_l}(\tau-1)+r_j(\tau);\linesspace
%\mbox{computes }\enc{r_i(\tau)}{j}; & \mbox{computes }\enc{r_j(\tau)}{i};\linesspace
\enc{s_k(\tau-1)}{j}\leftarrow \prreenc(\penc{s_k(\tau-1)}{k},\pdk{k}{j}); 
	& \enc{s_{_l}(\tau-1)}{i}\leftarrow \prreenc(\penc{s_{_l}(\tau-1)}{l},\pdk{l}{i}); \linesspace\\
		\multicolumn{2}{c}{
		\begin{array}{c}
%		\enc{n_i(\tau-1)+s_k(\tau-1)+r_i(\tau)}{j},~\enc{-r_i(\tau)}{i},~\penc{s_k(\tau-1)}{j},~d_i(\tau-1); \linesspace
		n_i(\tau-1)+s_k(\tau-1)+r_i(\tau),~\enc{s_k(\tau-1)}{j},~d_i(\tau-1); \\
		\varrightarrow{160}\linesspace
%		\enc{n_j(\tau-1)+s_{_l}(\tau-1)+r_j(\tau)}{j},~\enc{-r_j(\tau)}{j},~\penc{s_{_l}(\tau-1)}{i},~d_j(\tau-1); \linesspace
		n_j(\tau-1)+s_{_l}(\tau-1)+r_j(\tau),~\enc{s_{_l}(\tau-1)}{i},~d_j(\tau-1); \\
		\varleftarrow{160}
		\end{array}} \linesspace\\

%\mbox{decrypts }\enc{n_j(\tau-1)+s_{_l}(\tau-1)+r_j(\tau)}{i}; & \mbox{decrypts }\enc{n_i(\tau-1)+s_{_l}(\tau-1)+r_i(\tau)}{j};\linesspace

s_{_l}(\tau-1)\leftarrow\prdec(\enc{s_{_l}(\tau-1)}{i},\ppk{i}) & s_{k}(\tau-1)\leftarrow\prdec(\enc{s_{k}(\tau-1)}{j},\ppk{j})
\linesspace

%\mbox{decrypts }\penc{s_{_l}(\tau-1)}{i}; & \mbox{decrypts } \penc{s_k(\tau-1)}{j};\linesspace
\mbox{compute }n_j(\tau-1)+r_j(\tau); 				& \mbox{compute }n_i(\tau-1)+r_i(\tau);
\linesspace

lcm(\tau-1)\leftarrow\max(d_i(\tau-1),d_j(\tau-1)); & lcm(\tau-1)\leftarrow\max(d_i(\tau-1),d_j(\tau-1));
\linesspace

d_i(\tau)\leftarrow 2lcm(\tau-1); 					& d_j(\tau)\leftarrow 2lcm(\tau-1);
\linesspace


\mbox{compute }n_j(\tau)+obf_j(\tau) +s_i(\tau)\mbox{ as in Eq. (\ref{eq:update_step})}				& \mbox{compute }n_i(\tau)+obf_i(\tau) +s_j(\tau)\mbox{ as in Eq. (\ref{eq:update_step})}
\linesspace

\text{where:}											& \text{where:} 
\linesspace

\quad obf_j(\tau) = s_k(\tau-1)\frac{lcm(\tau-1)}{d_i(\tau-1)}+r_j(\tau)\frac{lcm(\tau-1)}{d_j(\tau-1)}; &  obf_i(\tau) = s_{_l}(\tau-1)\frac{lcm(\tau-1)}{d_j(\tau-1)}+r_i(\tau)\frac{lcm(\tau-1)}{d_i(\tau-1)}; \quad
\linesspace


% \mbox{\quad is computed as in eq. (\ref{eq:update_step}) where} & \mbox{is computed as in eq. (\ref{eq:update_step}) where\quad}\linesspace
% \quad obf_j(\tau)=s_k(\tau-1)\frac{lcm(\tau-1)}{d_i(\tau-1)}+r_j(\tau)\frac{lcm(\tau-1)}{d_j(\tau-1)}; & obf_i(\tau)=s_{_l}(\tau-1)\frac{lcm(\tau-1)}{d_j(\tau-1)}+r_i(\tau)\frac{lcm(\tau-1)}{d_i(\tau-1)};\quad\linesspace

\penc{s_i(\tau)}{i}\leftarrow \prenc_2(s_i(\tau),\ppk{i}); & \penc{s_j(\tau)}{j}\leftarrow \prenc_2(s_j(\tau),\ppk{j}); \linesspace%\\
	
	\multicolumn{2}{c}{
		\begin{array}{c}
		%		\enc{n_i(\tau-1)+s_k(\tau-1)+r_i(\tau)}{j},~\enc{-r_i(\tau)}{i},~\penc{s_k(\tau-1)}{j},~d_i(\tau-1); \linesspace
		n_j(\tau)+obf_j(\tau) +s_i(\tau),~\penc{s_i(\tau)}{i}; \\
		\varrightarrow{160}
		\linesspace
		%		\enc{n_j(\tau-1)+s_{_l}(\tau-1)+r_j(\tau)}{j},~\enc{-r_j(\tau)}{j},~\penc{s_{_l}(\tau-1)}{i},~d_j(\tau-1); \linesspace
		n_i(\tau)+obf_i(\tau) +s_j(\tau), ~\penc{s_j(\tau)}{j}; \\
		\varleftarrow{160}
		\end{array}}\\
	% \linesspace
\mbox{compute }obf_i(\tau); & \mbox{compute }obf_j(\tau);\linesspace
\mbox{compute }n_i(\tau)+s_j(\tau). & \mbox{compute }n_j(\tau)+s_i(\tau).


%\mbox{encrypts }n_j(\tau-1)+r_j(\tau)\mbox{ by using }\textit{PuK}_j; & \mbox{encrypts }n_i(\tau-1)+r_i(\tau)\mbox{ by using }\textit{PuK}_i;\\
%\mbox{compute }d_i(\tau-1),~\enc{n_i(\tau-1)}{j}\mbox{ as in eq. (\ref{eq:encrypted_step});} & \mbox{compute }d_j(\tau-1),~\enc{n_j(\tau-1)}{i}\mbox{ as in eq. (\ref{eq:encrypted_step});}\\
%\mbox{compute }\enc{n_i(\tau-1)+s_i(\tau)}{j}; & \mbox{compute }\enc{n_j(\tau-1)+s_j(\tau)}{i};\\
%		\multicolumn{2}{c}{
%		\begin{array}{c}
%		\enc{n_i(\tau-1)+s_i(\tau)}{j},~\enc{-s_i(\tau-1)}{b}~\forall b\in{\cal N}_j/\{i\};\\
%		\varrightarrow{80}\\
%\enc{n_j(\tau-1)+s_j(\tau)}{i},~\enc{-s_j(\tau)}{a}~\forall a\in{\cal N}_i/\{j\};\\
%		\varleftarrow{80}
%		\end{array}} \\
%\mbox{decrypts }\enc{n_j(k-1)+s_j(k)}{i}\mbox{ by using }\textit{PrK}_i; & \mbox{decrypts }\enc{n_i(k-1)+s_i(k-1)}{j}\mbox{ by using }\textit{PrK}_j;\\
%\mbox{encrypts }n_j(k-1)+s_j(k)\mbox{ by using }\textit{PuK}_a~\forall a\in{\cal N}_i/\{j\}; & \mbox{encrypts }n_i(k-1)+s_i(k-1)\mbox{ with }\textit{PuK}_b ~\forall b\in{\cal N}_j/\{i\};\\
%\mbox{compute }\enc{n_i(k-1)}{a}
% ~\forall a\in{\cal N}_i/\{j\}. &\mbox{compute }\enc{n_j(k-1)}{b}%=\enc{n_i(k-1)+s_i(k-1)}{a}\enc{-s_i(k-1)}{a} 
%~\forall b\in{\cal N}_j/\{i\}.
\end{array}
$$
}

